TriCheck: Memory Model Verification at the Trisection of Software, Hardware, and ISA

Memory consistency models (MCMs) which govern inter-module interactions in a shared memory system, are a significant, yet often under-appreciated, aspect of system design. MCMs are defined at the various layers of the hardware-software stack, requiring thoroughly verified specifications, compilers, and implementations at the interfaces between layers. Current verification techniques evaluate segments of the system stack in isolation, such as proving compiler mappings from a high-level language (HLL) to an ISA or proving validity of a microarchitectural implementation of an ISA. This paper makes a case for full-stack MCM verification and provides a toolflow, TriCheck, capable of verifying that the HLL, compiler, ISA, and implementation collectively uphold MCM requirements. The work showcases TriCheck's ability to evaluate a proposed ISA MCM in order to ensure that each layer and each mapping is correct and complete. Specifically, we apply TriCheck to the open source RISC-V ISA, seeking to verify accurate, efficient, and legal compilations from C11. We uncover under-specifications and potential inefficiencies in the current RISC-V ISA documentation and identify possible solutions for each. As an example, we find that a RISC-V-compliant microarchitecture allows 144 outcomes forbidden by C11 to be observed out of 1,701 litmus tests examined. Overall, this paper demonstrates the necessity of full-stack verification for detecting MCM-related bugs in the hardware-software stack.

==> 00-cppbackground.tex <==
\section{C++ Memory Model Background (keep?)}
\label{sec:cppbackground}
%An ISA can only effectively serve as an interface between hardware and software when it is precisely defined prior to being licensed or open-sourced to hardware designers.
%Most generally, MCMs specify the rules and guarantees governing the ordering and visibility of accesses to shared memory.
%Frequently regarded as the most intuitive MCM, Sequential Consistency (SC)~\cite{lamport:sc} classifies a program execution as \textit{sequentially consistent} if the result is the same as if all operations (from all cores) were executed in some global sequential order, and the operations of each individual core appear in this global sequence in the order specified by its corresponding program.
%While it is intuitive for programmers to reason about SC code, little to no software or hardware models are SC due to perceived performance penalties.
%In hardware, there have been many attempts at mitigating this cost, commonly leveraging techniques such as aggressive post-retirement speculation and rolling back execution in the case of a coherence violation~\cite{invisifence, bulksc, speculativesc, sc_ilp_rc, Ranganathan:speculativeretirement, Wenisch:storewaitfree}. Arguing that these designs are expensive in terms of hardware cost and complexity of cache coherence protocols, other techniques have been proposed that aim to enforce SC only for conflicting accesses~\cite{endtoendsc, efficientsc, atomicsc}.
%Nevertheless, single-core performance optimizations violate SC, and most manufactures have elected to build hardware with MCMs that relax SC~\cite{IBM370, TSO, PC, PSO, WO, RCsc, RCpc, Alpha, RMO, PowerPC}. 

%Exploits the observation that hardware need not enforce any memory model constraints on accesses to thread-local and shared read-only loactions. Our design employs an additional unordered store buffer for fast-tracking thread-local stores and allowing later memory accesses to proceed without a memory ordering related stall.~\cite{endtoendsc}
%Guarantee SC by completing conflicting memory operations, within and across processors, in an order consistent with program order. No post-retirement speculation or associated hardware costs. Use cache coherence protocol. When a write-miss is encountered, they conservatively estimate ~\cite{efficientsc}
%Attempts to reap the benefits of memory reference reordering in simple in-order processors without requirement any speculation or rollback support. Considerably less hardware resources and no coherence protocol modifications. Acquire and release a global mutex ~\cite{atomicsc}
%(1) maintain speculative state at a per-store granularity, causing storage requirements to grow proportionally to speculation depth, or (2) employ distributed global commit arbitra- tion using unconventional chunk-based invalidation mechanisms.~\cite{invisifence}
%Post-retirement speculation -- speculation beyond instruction window -- to eliminate program ordering stalls~\cite{invisifence, bulksc, speculativesc, sc_ilp_rc, Ranganathan:speculativeretirement, Wenisch:storewaitfree}
%These MCMs are often described with the adjectives ``strong'' or ``weak;'' however, Lustig et al. demonstrate that there is no guarantee that one MCM is strictly stronger or weaker than another~\cite{armor}.
%Single core performance optimizations contravene SC. 
%Complicated to implement and verify, but easy to program for.

%\subsection{Preserved Program Order}
%Coherence, Single Writer Multiple Reader (SWMR), Data Value Invariant (DVI), deadlock avoidance mechanisms~\cite{primer,ccicheck}. \\In coherence papers, total order on stores to the same address... 
%You can have coherence at the program level being per-location SC, but at the architecture level you could have -- Ghar defintion (1990). Also in primer -- Primer cites him.
%Discuss the parts of coherence. Total order on all stores to the same address. Everyone agrees on that order. Those writes are made visible to all cores in the same order.

%\subsection{Dependencies}
%\subsection{Store Atomicity}

%\subsection{Cumulativity}
%To restore the causality lost in the nMCA stores example of Section~\ref{sec:atomicity}, architectures such as ARM and Power implement cumulative fences that enforce orderings on access in threads other than the fencing thread~\cite{armor}. 
%It is difficult to precisely define cumulativity, and there are many proposed definitions~\cite{}.
%Fences are typically defined by specifying memory accesses that the fence is ordered after (i.e., group A) and that the fence is ordered before (i.e., group B). 
%AC is further subdivided into \textit{strong A-cumulativity} (sAC) and \textit{weak A-cumulativity} (wAC). sAC requires that before a given thread can observe an access in group B, it must first observe all accesses in group A. wAC requires that before a given thread can observe an access in group B, all threads must observe all accesses in group A.
%
%Referring again to Figure~\ref{fig:wrcassembly}, and the case where stores are nMCA, we can see a fence on C1 that is both wAC and BC is sufficient to prevent the non-SC outcome. The base cases for groups A and B are accesses \texttt{b} and \texttt{c}, respectively. Since \texttt{a} performed before the group A access, \texttt{a}, it is also in group A according to AC. Since \texttt{d} returns the value of the group B store, \texttt{c}, it is in group B according to BC. wAC ensures that before an access in group B (e.g., \texttt{d}) can observe the group B write, \texttt{c}, it must have observed all group A accesses. Group A includes \texttt{a}, and \texttt{e} may no longer read the stale value, 0.
%Cumulative orderings must be addressed whenever nMCA writes are permitted. Cumulativity will affect all instances where writes are to be ordered before another another memory or synchronization instruction.
    
\subsection{Copied over...FIXME}
    \textsc{C/C++ Atomics}: The ISA must provide instructions capable of enforcing the orderings required by the C/C++ atomic \texttt{memory\_order} primitives. At minimum, the ISA-level MCM should be able to support \texttt{sc} atomics, but increased performance will likely result when more fine-grained ISA synchronization instructions exist for implementing low-level (i.e., \texttt{acq} and \texttt{rel}) atomics.
    For architectures that permit nMCA stores, failure to address the wCA and sCA requirements of release-acquire synchronization and sequentially consistent orderings, respectively, can render the ISA unable to serve as a compiler for C/C++. 

\subsection{C/C++ HLL MCM Explained Through Examples}
The C/C++ MCM~\cite{cppconcurrency}, is a formal specification that defines the outcomes that are either \textit{permitted} or \textit{forbidden} for a given C/C++ program execution. This differs from ISA MCMs which define which outcomes are \textit{observable} or \textit{not observable} for a given instruction assembly sequence.
The  C/C++ HLL MCM features atomic variables with corresponding \texttt{memory\_order} identifiers:
\texttt{relaxed}  (\texttt{rlx}),
\texttt{consume}  (\texttt{con}),
\texttt{acquire}  (\texttt{acq}),
\texttt{release}  (\texttt{rel}), 
\texttt{acq\_rel} (\texttt{ar}), and \texttt{seq\_cst} (\texttt{sc}).
These identifiers may be applied to instructions that access memory or instructions that impose ordering constraints on memory access (i.e., fences), specifying how other memory accesses may be ordered with respect to the atomic operation they are assigned to.

Any atomic memory operation may be labeled \texttt{rlx}, which inflicts no additional ordering or synchronization constraints aside from being atomic.
Loads may be annotated with \texttt{acq} or \texttt{sc}, and stores with \texttt{rel} or \texttt{sc}. 
Read-modify-write (RMW) operations may be labeled \texttt{aq}, \texttt{rel}, \texttt{ar}, or \texttt{sc}. 
The default memory order of all atomic operations is \texttt{sc}. When this memory order is applied to a read, write, or RMW operation, the access behaves like an Acq, Rel, or AR operation, respectively. Additionally, in a given execution, there there exists a single, total order of \texttt{sc} operations on which all threads agree~\cite{batty:overhauling}.

To explain the semantics of these \texttt{memory\_order} primitives, we will show how they affect the allowable outcomes of the litmus tests in Figures~\ref{fig:wrc} and~\ref{fig:iriw}.
Figure~\ref{fig:wrc} depicts a C/C++ version of the assembly WRC litmus test in Figure~\ref{fig:wrcassembly}.
In the HLL model of C/C++, \texttt{rlx} stores are subject to the same ordering semantics as nMCA assembly stores. Therefore, even though the \texttt{acq} loads on T1 and T2 ensure PO order on those threads, the counter-intuitive non-SC outcome is permitted by the C/C++ HLL model by the same reasoning as the example in Section~\ref{sec:atomicity}.
If we change the memory order of access \texttt{c} to \texttt{rel}, we can weaken \texttt{b} to \texttt{rlx} (as shown in Figure~\ref{fig:wrcaqrl}) and render the outcome forbidden by the HLL MCM for the following reasons:
\begin{enumerate}
    \item Loads and stores are ordered \textit{before} \texttt{rel} stores, ensuring that \texttt{b} and \texttt{c} maintain PO.
    \item Loads and stores are ordered \textit{after} \texttt{acq} loads, ensuring that \texttt{d} and \texttt{e} maintain PO.
    \item \textit{Release-acquire synchronization }in the C/C++ HLL MCM ensures that when an \texttt{acq} load reads from a \texttt{rel} write, the thread performing the \texttt{acq} load is guaranteed to see everything that happened before the \texttt{rel} write. This this synchronization is analogous to the wAC and BC orderings of Section~\ref{sec:cumulativity}.
\end{enumerate}

Figure~\ref{fig:iriwrlx} is a C/C++ program that again demonstrates the nMCA behavior of C/C++ stores.
Accesses \texttt{a} and \texttt{b} perform independent stores that are then independently read in two different orders by T2 and T3.
The \texttt{acq} loads \texttt{c} and \texttt{e} guarantee that accesses following them (i.e., \texttt{d} and \texttt{f}, respectively), will execute in PO.
As in Figure~\ref{fig:wrcrlx}, it is possible that T2 and T3 see the updated values of \texttt{x} and \texttt{y} in different orders than one another. 
Changing \texttt{a} and \texttt{b} to \texttt{rel} stores, as depicted in Figure~\ref{fig:iriwaqrl}, still allows the non-SC outcome for the following reasons:
\begin{enumerate}
    \item Loads and stores are ordered \textit{after} the \texttt{acq} loads, ensuring that \texttt{c} and \texttt{d} maintain PO and \texttt{e} and \texttt{f} maintain PO.
    \item Release-acquire synchronization as described in the previous example is not enough to forbid the non-SC outcome in this case. Here we have two acquire-release pairs, \texttt{a}-\texttt{c} and \texttt{b}-\texttt{e}. Looking at the \texttt{a}-\texttt{c} pair first, \texttt{c} reads from \texttt{a} and therefore must see everything that happened before \texttt{a}. As there are no other stores before \texttt{a} in PO and no other loads before \texttt{a} in PO that could have witnessed another store, this acquire-release relationship does not enforce any additional orderings. The same is true for the \texttt{c}-\texttt{e} pair.
\end{enumerate}
In Figure~\ref{fig:iriwsc}, we assign the \texttt{sc} memory order to accesses \texttt{a}, \texttt{b}, \texttt{d}, and \texttt{f}. The \texttt{acq} loads from Figure~\ref{fig:iriwaqrl} remain; this is because an \texttt{sc} load behaves as an \texttt{acq} access, only ordering instructions after it in PO. The non-SC outcome is now forbidden due to the requirement there exists \textit{total order} on all \texttt{sc} atomic operations that all threads agree on.
This example demonstrates the difference between wAC and sAC.
%-- Current C/C++ concurrency model first described here\cite{cppconcurrency} \\
%-- Much work done to formalize mapping of C/C++ to weak hardware~\cite{} \\
%-- For C++ applications to run well, we need HW to implement C++ synchronization primitives well. For this reason C++ was designed to work well with %POWER/ARM and ARM has recently added acquire/release opcodes to their ISA to accommodate C++. \\
%-- Benefits of having acqure/release/acquire\_release fences? => performance. Rather than having an acquire sitting in a loop, we could have a relaxed %read in a loop followed by an acquire fence~\cite{POWERlrsc}.
%--If a program is ``properly labled'' language level, but the hardware does not correctly enforce the orderings required by the HLL memory order %primitives, the SC-for-DRF guarantees break
%--Mappings are important, particularly for performance critical data structures, e.g., work-steal queue and read-copy-update


%\textsc{RMW Atomicity}: There should be a mechanism for implementing atomic read-modify-write (RWM) operations. RMW atomicity is often achieved via compare-and-swap (CAS) or load-reserved and store-conditional (LR/SC) instructions~\cite{}.
%\item \textsc{No Limits}: The ISA specification should not be closely tied to, or place a mandate on, microarchitectural implementations of that model.
\begin{figure}[t]
\begin{center}
\centering
\small
\setlength\tabcolsep{4pt} % default value: 6pt
    \begin{tabular}{| c  c  c |}
    \hline
    \multicolumn{3}{|c|}{\textbf{Initial conditions}: x=0, y=0}\\ \hline
    T0            & T1            & T2            \\ \hline
   a: st(x,1,rlx) & b: r0 = ld(x,acq) & d: r1 = ld(y,acq) \\
                       & c: st(y,1,rlx) & e: r2 = ld(x,rlx) \\ \hline
    \multicolumn{3}{|c|}{\textbf{Allowed Non-SC Outcome}: r0=1, r1=1, r2=0}     \\
    \hline
    \end{tabular}
    \captionof{subfigure}{WRC with \texttt{rlx} loads stores.}
    \label{fig:wrcrlx}

    \vspace*{0.2 cm}

    \begin{tabular}{| c  c  c |}
    \hline
    \multicolumn{3}{|c|}{\textbf{Initial conditions}: x=0, y=0}\\ \hline
    T0            & T1            & T2            \\ \hline
    a: st(x,1,rlx) & b: r0 = ld(x,rlx) & d: r1 = ld(y,acq) \\
                       & c: st(y,1,rel) & e: r2 = ld(x,rlx) \\ \hline
    \multicolumn{3}{|c|}{\textbf{Forbidden Non-SC Outcome}: r0=1, r1=1, r2=0}     \\
    \hline
    \end{tabular}
    \captionof{subfigure}{WRC where the variable \texttt{y} is accessed by an \texttt{aq} load on T1 and a \texttt{rl} store on T2. All other accesses are \texttt{rlx} accesses.}
    \label{fig:wrcaqrl}
\end{center}
\caption{Variations of the HLL Write-to-Read Causality (WRC) litmus test that demonstrate the affects of the C/C++ \texttt{acq} and \texttt{rel} memory orders. T0, T1, and T2, represent three unique C/C++ threads.}
\label{fig:wrc_old}
\end{figure}


\begin{figure}[t]
\begin{center}
\begin{minipage}{.5\textwidth}
\centering
\small
\setlength\tabcolsep{4pt} % default value: 6pt
    \begin{tabular}{| c  c  c  c |}
    \hline
    \multicolumn{4}{|c|}{\textbf{Initial conditions}: x=0, y=0}\\ \hline
    T0            & T1            & T2            & T3    \\ \hline
    a: st(x,1,rlx) & b: st(y,1,rlx) & c: r0 = ld(x,acq) & e: r2 = ld(y,acq) \\
                    &                    & d: r1 = ld(y,rlx) & f: r3 = ld(x,rlx) \\ \hline
    \multicolumn{4}{|c|}{\textbf{Allowed Non-SC Outcome}: r0=1, r1=1, r2=0, r3=0}     \\
    \hline

    \end{tabular}
    \captionof{subfigure}{IRIW with \texttt{rlx} loads and stores.}
    \label{fig:iriwrlx}

    \vspace*{0.2 cm}
    
    \begin{tabular}{| c  c  c  c |}
    \hline
    \multicolumn{4}{|c|}{\textbf{Initial conditions}: x=0, y=0}\\ \hline
    T0            & T1            & T2            & T3    \\ \hline
    a: st(x,1,rel) & b: st(y,1,rel) & c: r0 = ld(x,acq) & e: r2 = ld(y,acq) \\
                    &                    & d: r1 = ld(y,rlx) & f: r3 = ld(x,rlx) \\ \hline
    \multicolumn{4}{|c|}{\textbf{Allowed Non-SC Outcome}: r0=1, r1=1, r2=0, r3=0}     \\
    \hline

    \end{tabular}
    \captionof{subfigure}{IRIW with \texttt{rel} stores, and two \texttt{acq} loads.}
    \label{fig:iriwaqrl}

    \vspace*{0.2 cm}

    \begin{tabular}{| c  c  c  c |}
    \hline
    \multicolumn{4}{|c|}{\textbf{Initial conditions}: x=0, y=0}\\ \hline
    T0            & T1            & T2            & T3    \\ \hline
    a: st(x,1,sc) & b: st(y,1,sc) & c: r0 = ld(x,acq) & e: r2 = ld(y,acq) \\
                    &                    & d: r1 = ld(y,sc) & f: r3 = ld(x,sc) \\ \hline
    \multicolumn{4}{|c|}{\textbf{Forbidden Non-SC Outcome}: r0=1, r1=1, r2=0, r3=0}     \\
    \hline

    \end{tabular}
    \captionof{subfigure}{IRIW with \texttt{sc} stores, two \texttt{sc} loads, and two \texttt{acq} loads.}
    \label{fig:iriwsc}
  
\end{minipage}%
\end{center}
\caption{Variations of the HLL Independent Reads of Independent Writes (IRIW) litmus test that demonstrate the affects of the C/C++ \texttt{sc} memory orders. T0, T1, and T2, represent three unique C/C++ threads.}
\label{fig:iriw}
\end{figure}




==> 07-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{ISA Specifications Should Be General}
The ISA specification should be designed such that it does not constrain high performance microarchitectural implementations. For example, while nMCA store behavior is often explained using shared write-through caches or store buffers; however, this is not the only scenario in which this type of behavior might arise. We demonstrate this in the A9 $\mu$Spec Base and Base~+~A models.
Additionally, requiring all acquire, release, and sequentially consistent accesses to be implemented with RMW operations is unnecessarily restrictive. In the case of a no-write-allocate cache and RMW release operations, you must bring data into your cache unnecessarily. If release operations were implemented as writes, there would be no need to pollute cache on a release write miss.

\subsection{Load-Reserved and Store-Conditional}
The Base~+~A RISC-V MCM provides support for complex RMW operations with LR/SC instructions. LR/SC sequence, like AMOs, may be given acquire, release, or sequentially consistent ordering semantics for implementing C11 atomics.
The manual indicates that the sequence can be given \textit{acquire semantics} by setting the \textit{aq} bit on the SC instruction, \textit{release semantics} by setting the rl bit on the LR instruction, and sequentially consistent semantics by setting both\textit{aq} and \textit{rl} bits on the LR instruction the \textit{aq} bit on the SC instruction.

This is counter-intuitive given Gharachorloo et. al's first formulation of release consistency which , which the RISC-V manual cites itself. In this first presentation of release consistency, an acquire access is performed to gain access to a set of shared locations and \textit{always a read} of a shared location.  A release access on the other hand is an unlock operation or a process of setting a flag and is \textit{always a write} to a shared location. RMW operations function as acquire accesses by annotating the read as an acquire (the most common scenario. To guarantee release and acquire semantics, the write can additionally be labeled as a release access~\cite{gharachorloo:release}. \undrline{Our recommendation} is that only loads should be able to function as acquires and only stores should be able to function as release. Additionally, we think that it is unnecssarily restritive to only provide acquire, release, and sequentially consistent semantics for RMW operations.



==> background.tex <==
\section{Background on Memory Consistency Models}
%\label{sec:background}
%\subsection{Spectrum of Memory Consistency Models}

\subsection{Release Consistency and its Many Variants}
Release consistency represents a class of memory models that aim to provide relatively intuitive outcomes for programs that are properly synchronized.
Release consistency was first proposed with two variants, RCsc and RCpc~\cite{gharachorloo:release}.\\
--Compiler optimizations in the synchronized regions of properly synchronized programs. \\
--A modern and well-studied example of release consistency is the C/C++ HLL model. Through the --SC-for-DRF paradigm, sequentially consistency semantics are guaranteed for properly synchronized programs. \\
--This model has seemingly inspired other variants of release consistency to emerge, including AMRv8 \\
--Intuition behind acquire and release; Ghar(1990 paper or thesis), gaining access to a region, releasing access
--While SC-for-DRF is an attractive paradigm, it can only be effective if MCMs are carefully specified and all translation interfaces are implemented correctly~\cite{commoncompiler}.

In software, as a compromise between programmability and aggressive performance optimizations in compilers and hardware, the SC-for-DRF (i.e., Sequential Consistency for Data Race Free) programming paradigm guarantees sequentially consistent semantics for properly synchronized programs~\cite{weakordering}. However, this still requires that the underlying synchronization primitives are correctly implemented in hardware. This in turn necessitates an ISA specification that clearly defines what compiler writers can expect from the hardware and what hardware designers must provide.




==> motivating.tex <==
\section{Weak Memory Models: What Can Go Wrong?}
\label{sec:motivating}
\subsection{ARM Read-after-Read Hazard}
Upon acknowledging the read-after-read hazard discussed in Section~\ref{sec:intro}, ARM issued a workaround affecting both compilers and hand-tuned assembly code. In \cite{ARMHazard}, they acknowledge that due to the vast amount of load instructions, binary patching in the linker is infeasible. Furthermore, as this issue only affects C/C++ \textit{atomic} and \textit{volatile} variables, it is wasteful to require this ordering for all program-order (PO) same-address loads. Therefore, they suggest that compilers are rewritten to issue an ARM \texttt{dmb} fence instruction immediately following susceptible loads. Programmers must also manually fix all in-line assembly.

We believe there are important lessons to be learned from the ARM read-after-read hazard. Firstly, a compiler fix is dependent upon the existence of an instruction that is in fact semantically cable of restoring the desired ordering that is not enforced by hardware. This instruction (\texttt{dmb ish} in this example) must also be properly implemented in the microarchitecture. Further, injecting instructions into a program to enforce desired orderings can result in significantly reduced performance, particularly if the only instruction available to enforce the orderings in question is stronger than required. Lastly, in some cases, recompilation may be infeasible, leaving us subject to the performance costs of DBI-style solutions.

%ARM acknowledges this as a bug in 2011 and we can still see this today. Many phones.
%We measured the performance penalty of statically inserting \texttt{dmb ish} barriers...
%Using the litmus test (i.e., a small parallel program used to exercise the behaviors of an MCM) depicted in Figure~\ref{fig:co-rsdwi} and the \textit{litmus} utility from the \textit{Herd} tool suite~\cite{alglave:herd} we generated a testing harness to repeatedly execute the two-thread code segment on ARM/Android hardware. Doing so, we were able to observe the read-to-read reordering hazard on a Samsung Galaxy Nexus and (list other phone(s)?).

\subsection{Cost to Prevent Read-after-Read Hazard}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/dmboverhead.pdf}
  \caption{Overhead of inserting fences to prevent read-after-read hazard for parallel Sieve of Eratosthenes variant from \cite{evil} on a Samsung Galaxy S7}
  \label{fig:dmboverhead}
\end{figure}

In order to approximate the cost of preventing the read-read hazard for applications that make significant use of relaxed atomics, we used variants of the parallel version of the sieve of Eratosthenes from \cite{evil}. The main loop of the program is shown below.

\begin{verbatim}
for (my_prime = start; my_prime < SQRT;
    ++my_prime)
    if (!get(my_prime)) {
        for (multiple = my_prime;
                multiple < MAX;
                multiple += my_prime)
            if (!get(multiple)) set(multiple);
}
\end{verbatim}

%The parallel sieve consists of multiple threads operating on an array of size MAX of Boolean values, where each entry in the array represents a number in the range [0, MAX). At the start of the algorithm, all entries in the array are unset. Given a starting index i, a thread sets the multiples of each unset entry in the range [i, sqrt(MAX)). If a thread finds that an entry in this range is already set, it does not set the multiples of the entry because they will be set by another thread or as the multiples of another number. As a result, the program finishes quicker if more threads are running concurrently. (Note that when setting multiples, our version of the code only sets the multiple if it has not already been set.) At the end of the execution, the unset entries in the range [sqrt(MAX), MAX) are the prime numbers in that range. This algorithm is similar to the one used for mark bit handling in a parallel mark-sweep garbage collector~\cite{evil}.

The parallel sieve application gives the same results regardless of whether or not there is any synchronization between threads in the \texttt{get(..)} and \texttt{set(..)} calls. Thus, the \texttt{get(..)} and \texttt{set(..)} calls can be implemented with either relaxed atomics or sequentially consistent atomics without compromising correctness.

We implemented three variants of the parallel sieve algorithm. The first variant uses relaxed atomics to implement \texttt{get(..)} and \texttt{set(..)}. The second variant uses relaxed atomics but with a \texttt{dmb ish} fence added after the relaxed load in \texttt{get(..)}, in accordance with ARM's recommended fix to prevent the load-load hazard on Cortex-A9 processors~\cite{ARMHazard}. The third variant uses sequentially consistent atomics, implemented using a combination of regular loads and stores and \texttt{dmb ish} fences, as \cite{sewell:mappings} recommends for ARMv7 processors.

We ran the variants of the parallel sieve application with a \texttt{MAX} value of $10^8$ on a Samsung Galaxy S7 with an Exynos 8890 8-core processor, varying the number of threads between 1 and 32. The results of our experiments are shown in Figure~\ref{fig:dmboverhead}.

The variant using relaxed atomics finishes fastest, as its \texttt{get(..)} and \texttt{set(..)} calls contain no fences to constrain execution. The variant with the load-load hazard fix is always slower than the relaxed atomic variant due to the extra \texttt{dmb ish} fence. The overhead of the fix is 20.3\% additional execution time on average. Furthermore, the performance of the fixed variant degrades to the level of fully sequentially consistent atomics for thread counts over 13. This experiment indicates that the overhead of fixing the load-load hazard can be quite significant for applications that liberally use relaxed atomics.

\subsection{Subtlities of Weakening Features of MCMs}
Referring back to the features of MCMs discussed in Section~\ref{sec:background}, there are various issues that can arise when the weakening of these features is not carefully considered at ISA Design time. Here, we enumerate some potential issues:
\begin{enumerate}
    \item \textsc{Preserved Program Order}: When defining PPO, designers should explicitly specify orderings that apply to sets of memory operations with the \textit{same address} and \textit{different addresses}, respectively. Failure to do so has resulted in forbidden, yet observable, reordering of reads of the same address on some GPU sand some ARM implementations as discussed in Section~\ref{sec:intro} ~\cite{gpuconcurrency, alglave:herd}.
    \item \textsc{Dependencies}: Martin et.al~\cite{Martin:valueprediction} demonstrate that value prediction allows a processor to relax the ordering between data dependent operations, and that verifying value prediction by comparing the predicted and actual values is not sufficient in a multi-core environment.
    They present a pointer-manipulation example with two-element linked list. The \textit{Head} pointer initially points to element \textit{A}. The \textit{Writer} thread writes some data to element \textit{B} before subsequently updating \textit{Head} to point to \textit{B}. Meanwhile, the \textit{Reader} thread, predicts that \textit{Head} points to \textit{B} and loads stale data from \textit{B} before the writing thread has updated the value.
    When the value prediction is later resolved, the \textit{Reader} thread confirms its prediction was correct but has loaded stale data. 
    \item \textsc{Store Atomicity}: In this case, the system allows nMCA stores and effectively allows the reordering of the write on C0 with the write on C1 from the viewpoint of C2, despite their causal relationship as domonstrated in Figure~\ref{fig:wrcassembly}.
    \item \textsc{Safety Net}: Furthermore, there should be a ``safety net'' instruction or mechanism capable of restoring sequential consistency.
    As explained in Section~\ref{sec:motivating}, the ARM read-after-read hazard could be fixed in the compiler \textit{only} because an instruction existed in the ISA that was capable of restoring the unenforced ordering. An ISA instruction capable of bringing all cores up to a mutual point in logical time provides a safety net for correctness in all cases. If nMCA writes are permitted, this instruction must enforce cumulative orderings.
    \item \textsc{C/C++ Atomics}: The ISA must provide instructions capable of enforcing the orderings required by the C/C++ atomic \texttt{memory\_order} primitives. At minimum, the ISA-level MCM should be able to support \texttt{sc} atomics, but increased performance will likely result when more fine-grained ISA synchronization instructions exist for implementing low-level (i.e., \texttt{acq} and \texttt{rel}) atomics.
    For architectures that permit nMCA stores, failure to address the wCA and sCA requirements of release-acquire synchronization and sequentially consistent orderings, respectively, can render the ISA unable to serve as a compiler for C/C++. 
\end{enumerate}

%\begin{figure*}[h]
%  \includegraphics[width=\textwidth, center]{figures/motivatingexample.png}
%  \caption{}
%  \label{fig:motivating}
%\end{figure*}

%\begin{figure*}[ht]
%  \label{ fig7} 
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%    \includegraphics[width=.8\linewidth]{figures/coRSDWIcpp.png}
%    \captionsetup{width=0.95\textwidth}
%    \captionof{subfigure}{In this C++ program, all memory operations are \texttt{memory\_order\_relaxed}, indicating there is no special synchronization to constrain the execution.} 
%    \label{fig:corsdwicpp}
%    \vspace{2ex}
%  \end{minipage}%%
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%    \includegraphics[width=1.1\linewidth]{figures/coRSDWIcppCohcycle.png}
%    \captionsetup{width=0.95\textwidth}
%    \captionof{subfigure}{Using the axioms of \textbf{Definition 11} from \cite{batty:overhauling}, we analyze the memory accesses of the C++ program in Figure~\ref{fig:corsdwicpp} to determine if stated outcome is allowed by the C/C++ HLL MCM. We omit a full set of relations for clarity, but demonstrate that the Coh axiom is violated for this execution, thereby forbidding the stated outcome.} 
%    \label{fig:corsdwicppcycle}
%    \vspace{2ex}
%  \end{minipage} 
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%    \includegraphics[width=.6\linewidth]{figures/coRSDWIARM.png} 
%    \captionsetup{width=0.95\textwidth}
%    \captionof{subfigure}{We draw the happens-before edges~\cite{} that correspond to the outcome forbidden by the C/C++ HLL MCM in Figure~\ref{fig:corsdwicppcycle} and show that the lack of ordering between the two highlighted loads on Core 0 causes the C/C++-forbidden outcome to be come \textbf{observable}.}
%    \label{fig:corsdwiarm}
%  \end{minipage}%% 
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figures/coRSDWIandroid.png} 
%    \captionsetup{width=0.95\textwidth}
%    \captionof{subfigure}{Result of iteratively running the ARM assembly program in Figure~\ref{fig:corsdwiarm} on a Galaxy Nexus 6, containing a Snapdragon 805~\cite{}. The number of times (63/10,000,000) varies from run to run.}
%  \end{minipage}
%  \caption{This example demonstrates how the lack of ordering between subsequent reads of the same address causes a C/C++ program to produce an output that is illegal according to the C/C++ HLL MCM specification. Even if a MCM is formally defined at the program level, its ordering primitives must be accuratly implimented by ISA instructions to prohibit erroneous results.}
%  \label{fig:motivating}
%\end{figure*}

% If the ISA required ordering between loads to same address, a cycle would be introduced into the execution graph rendering the illegal outcome unobservable.
%\begin{figure*}[!htb]
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{figures/coRSDWIcpp.png}
%  \label{fig:coRSDWIcpp}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{figures/coRSDWIARM.png}
%  \label{fig:coRSDWIARM}
%\endminipage\hfill
%\minipage{0.32\textwidth}%
%  \includegraphics[width=\linewidth]{figures/coRSDWIandroid.png}
%  \label{fig:coRSDWIandroid}
%\endminipage
%
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{figures/coRSDWIcpptemp.png}
%  \label{fig:coRSDWIARM}
%\endminipage\hfill
%\minipage{0.32\textwidth}%
%  \includegraphics[width=\linewidth]{figures/coRSDWIARMtemp.png}
%  \label{fig:coRSDWIARM}
%\endminipage
%\label{fig:motivating}
%\caption{motivating Example}
%\end{figure*}








==> oldcasestudy.tex <==
\section{Applying our Methodology to RISC-V}
\label{sec:casestudy}
%\label{sec:casestudy}
%\begin{table}
%\begin{center}
%\begin{tabular}{| l | l |}
% \hline
% STB        & Cores buffer stores                       \\ \hline
% byp        & Allow a Ld to commit if there is not      \\
%            & a St in the STB to the same address       \\ \hline
% coalesce   & Allow stores to coalesce in the STB       \\ \hline
% ROWE       & Read Own Write Early: Allow an Ld with a  \\
%            & corresponding St in the STB to complete by\\
%            & forwarding the pending value              \\ \hline
% IRIW       & Independent Reads Indipendent Writes (or  \\
%            & Read Others' Writes Early): STB may be    \\
%            & shared with one ore more other cores      \\ \hline
% LDB        & Cores buffer loads                        \\
% \hline
%\end{tabular}
%\end{center}
%\caption{caption here}
%\label{table:relaxationkey}
%\end{table}

We divide our case study into two halves, corresponding to each one of the Base and Base~+~A RISC-V ISAs. 
For each of these ISA specifications, we apply the iterative design and refinement methodology of Figure~\ref{fig:method}. 
Throughout our refinement process, we quantify the effects various compiler, ISA MCM specification, and $\mu$Spec refinements on whether produce hardware executions (methodology Step~\ref{item:operational}) that are \textit{stricter than}, \textit{weaker than}, on \textit{equivalent to} (methodology Step~\ref{item:equivalence}) the executions permitted by C/C++ HLL model (methodology Step~\ref{item:axiomatic}).

As laid out in Steps~\ref{item:inputs} and ~\ref{item:refinement} of Section~\ref{sec:method}, our toolflow uses three initial input components that my be subsequently iteratively modified. The initial inputs for our Base (resp. Base~+~A) evaluation are the Base (resp. Base~+~A) compiler mappings of Table~\ref{table:compilermappings}, the current Base (resp. Base~+~A) RISC-V ISA MCM specification, and a RISC-V microarchitectural implementation, modeled in $\mu$Spec, that is much stricter in terms of MCM optimizations than the current RISC-V Base (resp. Base~+~A) MCM specification requires. This, and other implemented $\mu$Spec models are described in Section~\ref{sec:microimplmentations}.

\subsection{Microarchitectural Implementations}
\label{sec:microimplmentations}
Throughout out our iterative refinement process, we modeled many RISC-V processor designs with varying levels of microarchitectural optimization.
The initial stricter-than-required $\mu$Spec design (for both Base and Base~+~A) is a pipeline resembling Rocket Chip~\cite{rocketchip}, a 6-stage in-order pipeline that implements the Base RISC-V ISA as well as some optional extensions, including the Atomics extension discussed in Section~\ref{sec:riscv}.
Step~\ref{item:refinement} indicates that any combination of compiler mappings, ISA MCM specification, or $\mu$Spec model, may be refined at the end of one iteration/start of another. On all iterations of our toolflow that involved a $\mu$Spec model refinement, all refinements resulting in microarchitectural ``weakenings'' were legal according to the current RISC-V ISA MCM specification.

\begin{table}
\begin{center}
\centering
\small
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{| l | c | c | c | c | c | c |}

 \cline{2-7}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Relaxed PO}} & \multicolumn{3}{c|}{\textbf{Store Atomicity}} \\ \hline
 \multicolumn{1}{|l|}{\textbf{RISC-V Model}} & W$\rightarrow$R & W$\rightarrow$W & R$\rightarrow$M & MCA & rMCA & nMCA \\ \hline
 WR+MCA     & \cm   &       &       & \cm   &       &       \\ \hline
 WR+rMCA    & \cm   &		&       &       & \cm   &       \\ \hline
 WM+rMCA	& \cm   & \cm   &       &       & \cm   &       \\ \hline
 MM+rMCA	& \cm	& \cm	& \cm   &       & \cm   &       \\ \hline
 WR+nMCA    & \cm   &       &		&       & \cm   & \cm   \\ \hline
 MM+nMCA    & \cm	& \cm   & \cm	&       & \cm	& \cm   \\ \hline
 Rocket-A9  & \cm	& \cm   & \cm	&       & \cm	& \cm   \\ 

 \hline
 
\end{tabular}
\end{center}
\caption{RISC-V $\mu$Spec models constructed by relaxing various aspects of PO and store atomicity from a baseline model resembling the RISC-V Rocket Chip~\cite{rocketchip}. All relaxations are legal according to the RISC-V ISA Manual~\cite{RISCV}. R, W, and M, correspond to read accesses, write accesses, and memory accesses (reads or writes), respectively. We note that these models exercise optimizations analogous to those presented in~\cite{adve:tutorial}.}
\label{table:relaxations}
\end{table}

Table~\ref{table:relaxations} summarize the spectrum of RISC-V-allowed relaxations that we exploited in our refinement process for both halves of our evaluation. As the RISC-V ISA does not distinguish between same address and different address memory instruction orderings, we do not distinguish a difference in this table.
Initially, all relaxations were implemented by adding various combinations of memory access buffers after the Commit stage in the Rocket Chip pipeline. We achieve the relaxation combinations of Table~\ref{table:relaxations} as follows:
\begin{enumerate}
    \item \textbf{WR+MCA}: W$\rightarrow$R reordering is achieved by buffering stores in a FIFO queue prior to being eventually pushed out to the rest of the memory hierarchy. Younger loads may continue past pending stores as long as the load address does not match the address of a pending store in the store buffer. Whenever there is a match, the load must wait for the corresponding store (and any prior stores, due to the FIFO property of the queue) to reach the memory hierarchy before it can load any data. No core can read writes early, so stores are MCA.
    \item \textbf{WR+rMC}: Builds on WR+MCA by allowing the store buffer to forward values pending store values to later loads of the same address. Later loads my proceed past earlier stores, regardless of their effective addresses. Stores preform once locally and again globally, rendering them rMCA.
    \item \textbf{WM+rMCA}: Extends WR+rMCA by allowing writes (to diffrent addresses) to retire from the store buffer out of order. Coherence requires a total global order on stores to the same address.
    \item \textbf{MM+rMCA}: Extends MM by allowing reads to commit out of order with earlier reads or writes. We maintain that read$\rightarrow$write ordering must be maintained for same address reads and writes, but we allow reordering for all read$\rightarrow$read pairs as the specification does not specify any particular ordering semantics for reads of the same address.
    \item \textbf{WR+nMCA}: Extends WR+rMC by allowing cores to share store buffers. This is analogous to the shared write-through cache scenario of \cite{cppconcurrency}, and enables nMCA stores.
    \item \textbf{MM+nMCA}: Extends MM+rMCA by allowing shared store buffers in the same vein as WR+nMCA.
    \item \textbf{Rocket-A9}: To demonstrate that the intricacies of nMCA stores do not depend on a design that contains a shared buffer or shared write-through cache, we model another microarchitecture with ISA-visible relaxations that match those of MM+nMCA. This time we leverage the ability of $\mu$Check to model the subtlties that can arise a the cache-coherence-consistency interface. To implement nMCA stores, this model features a write-back cache that allows multiple requests for write permission (for different addresses) to be in progress at the same time and a non-stalling directory protocol that allows the storing core to forward the store's value to another core before it has received all invalidations for the access. In this scenario, coherence is preserved, but nMCA stores arise~\cite{}.
    \textbf{TODO}: Mention SWMR and DVI? Or desribe \textit{why} coherence is preserved?
\end{enumerate}

\subsection{Iterative Refinement for RISC-V}
We began both halves of our analysis by modeling the WR+MCA design of Table~\ref{table:relaxations} in $\mu$Check.
The Base version of WR+MCA implements only the instructions present in the RISC-V Base ISA, including memory operations and fences of all relevant granularities.
The Base~+~A version expands upon the Base version, which additionally featuring \texttt{acq}, \texttt{rel}, and \texttt{sc} operations~\footnote{We refer to RISC-V Base~+~A operations that use both \texttt{acq} and \texttt{rel} instruction encoding bits as \texttt{sc} operations since they require a total SC order on which all threads agree}.

As required by Step~\ref{item:ctests} of our methodology, we gathered a set of C/C++ litmus tests capable of exercising various aspects PO and store atomicity and formatted these tests as templates where all atomic \texttt{memory\_orders} were replaced with placeholders. Using these templates, we generated a suite of litmus tests that featured all possible combinations of \texttt{rlx}, \texttt{acq}, \texttt{rel}, and \texttt{sc} \texttt{memory\_order} primitives for each place-holder (i.e., \texttt{C~Tests}).  Per Step~\ref{item:axiomatic}, we ran the suite of \texttt{C Tests} on the C/C++ Herd model~\cite{batty:overhauling} to determine the outomces \textit{permitted} and \textit{forbidden} by the C/C++ HLL MCM.
The Base (resp. Base~+~A) half of our analysis began by translating the \texttt{C~Tests} into their Base (resp. Base~+~A) RISC-V equivalents as specified in Step~\ref{item:compilation} via the compiler mappings in Table~\ref{table:compilermappings} to generate \texttt{Base Tests} (rexp. \texttt{Base+A Tests}).
%Upon comparing the results of the C/C++-required outcomes with the results of the \texttt{Base Tests} and \texttt{Base+A Tests} (presented in Section~\ref{sec:results}), we made a series of modifications to correct bugs in the current RISC-V MCM that prevent accurate compilation from C/C++ and to make this translation more optimal. These modifcations are laid out in Table~\ref{table:riscvflavors}.


\subsubsection{Base ISA Iterative Refinement}
We conducted the following iterations of refinement for the Base RISC-V ISA:
\begin{enumerate}
    \item \textbf{Inputs}: Base ISA~\cite{RISCV};
    Base compiler mappings (Table~\ref{table:compilermappings}); and
    Base WR+MCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to WR+rMCA

    \item \textbf{Inputs}: Base ISA;
    Base compiler mappings; and
    Base WR+rMCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to WM+rMCA

    \item \textbf{Inputs}: Base ISA;
    Base compiler mappings; and
    Base WM+rMCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to MM+rMCA
    
    \item \textbf{Inputs}: Base ISA;
    Base compiler mappings; and
    Base MM+rMCA $\mu$Spec model
    
    \textbf{Refinement}: Base ISA specification \textit{and} Base MM+rMCA $\mu$Spec model both refined to disallow  R$\rightarrow$R  reordering of reads to the same address
 
    \item \textbf{Inputs}: Base ISA refined to disallow R$\rightarrow$R reordering of reads to the same address;
    Base compiler mappings; and
    Base MM+rMCA $\mu$Spec model that disallows  R$\rightarrow$R  reordering of reads to the same address
    
    \textbf{Refinement}: $\mu$Spec model partially relaxed and partially strengthened to achieve WR+nMCA
    
    \item \textbf{Inputs}:  Base ISA refined to disallow R$\rightarrow$R reordering of reads to the same addres;
    Base compiler mappings; and
    Base WR+nMCA $\mu$Spec model

    \textbf{Refinement}: Refine ISA specification to include cumulative versions of fences for f[w,r], f[w,w], f[w,m], and f[m,m]; modify Base compiler mappings of Table~\ref{table:compilermappings} to use these new cumulative fences, update WR+nMCA $\mu$Spec model to implement these new fence types
  
    \item \textbf{Inputs}: Base refined to disallow R$\rightarrow$R reordering of reads to the same address \textit{and} to include cumulative fences;
    Base compiler mappings modified to use these new cumulative fences; and 
    WR+nMCA $\mu$Spec model that implements cumulative fence types
  
    \textbf{Refinement}: $\mu$Spec model relaxed further to MM+nMCA
  
    \item \textbf{Inputs}: Base refined to disallow R$\rightarrow$R reordering of reads to the same address \textit{and} to include cumulative fences;
    modified Base compiler mappings that use these new cumulative fences; and 
    MM+nMCA $\mu$Spec model that disallows R$\rightarrow$R reordering of reads to the same address \textit{and} implements cumulative fence types
  
    \textbf{Refinement}: Done
\end{enumerate}

\subsubsection{Base + A ISA Iterative Refinement}
We conducted the following iterations of refinement for the Base~+~A RISC-V ISA:
\begin{enumerate}
    \item \textbf{Inputs}: Base~+~A ISA~\cite{RISCV};
    Base~+~A compiler mappings (Table~\ref{table:compilermappings}; and
    Base~+~A WR+MCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to WR+rMCA

    \item \textbf{Inputs}: Base~+~A ISA;
    Base~+~A compiler mappings; and 
    Base~+~A WR+rMCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to WM+rMCA

    \item \textbf{Inputs}: Base~+~A ISA;
    Base~+~A compiler mappings; and 
    Base~+~A WM+rMCA $\mu$Spec model 
    
    \textbf{Refinement}: $\mu$Spec model relaxed further to MM+rMCA
    
    \item \textbf{Inputs}: Base~+~A ISA; 
    Base~+~A compiler mappings; and 
    Base~+~A MM+rMCA $\mu$Spec model
    
    \textbf{Refinement}: Base~+~A ISA specification \textit{and} Base~+~A MM+rMCA $\mu$Spec model both refined to disallow  R$\rightarrow$R  reordering of reads to the same address
 
    \item \textbf{Inputs}: Base~+~A ISA refined to disallow R$\rightarrow$R reordering of reads to the same address; 
    Base~+~A compiler mappings; and 
    Base~+~A MM+rMCA $\mu$Spec model that disallows  R$\rightarrow$R  reordering of reads to the same address
    
    \textbf{Refinement}: $\mu$Spec model partially relaxed and partially strengthened to achieve WR+nMCA
    
    \item \textbf{Inputs}:  Base~+~A ISA refined to disallow R$\rightarrow$R reordering of reads to the same address; 
    Base~+~A compiler mappings; and 
    Base~+~A WR+nMCA $\mu$Spec model

    \textbf{Refinement}: Refine Base~+~A compiler mappings of Table~\ref{table:compilermappings} to map \texttt{ld acq} to AMO.aq.rl and \texttt{st rel} to AMO.aq.rl
  
    \item \textbf{Inputs}:  
    Base~+~A ISA refined to disallow R$\rightarrow$R reordering of reads to the same address; 
    Base~+~A compiler mappings refined to map \texttt{ld acq} to AMO.aq.rl and \texttt{st rel} to AMO.aq.rl, and Base~+~A WR+nMCA $\mu$Spec model

    \textbf{Refinement}: Refine Base~+~A ISA to require release-acquire synchronization and the associated aspect of wAC \textit{and} add AMO.aq.sc and AMO.rl.sc instructions that behave like AMO.aq.rl but act as one-way barriers in their respective threads,  and refine Base~+~A compiler mappings to to map \texttt{ld acq} to AMO.aq, \texttt{st rel} to AMO.rl, \texttt{ld sc} to AMO.aq.sc, and \texttt{st sc} to AMO.rl.sc
  
    \item \textbf{Inputs}: Base~+~A ISA refined to disallow R$\rightarrow$R reordering of reads to the same address, to require release-acquire synchronization and the associated aspect of wAC, and to include AMO.aq.sc and AMO.rl.sc instructions;
    Base~+~A compiler mappings refined to map \texttt{ld acq} to AMO.aq, \texttt{st rel} to AMO.rl, \texttt{ld sc} to AMO.aq.sc, and \texttt{st sc} to AMO.rl.sc; and
    Base~+~A WR+nMCA $\mu$Spec model that implements new AMO.aq, AMO.rl, AMO.aq.sc, and AMO.rl.sc. instructions
  
    \textbf{Refinement}: $\mu$Spec model relaxed further to MM+nMCA
  
    \item \textbf{Inputs}: Base~+~A ISA refined to disallow R$\rightarrow$R reordering of reads to the same address, to require release-acquire synchronization and the associated aspect of wAC, and to include AMO.aq.sc and AMO.rl.sc instructions;
    Base~+~A compiler mappings refined to map \texttt{ld acq} to AMO.aq, \texttt{st rel} to AMO.rl, \texttt{ld sc} to AMO.aq.sc, and \texttt{st sc} to AMO.rl.sc; and
    Base~+~A MM+nMCA $\mu$Spec model that implements new AMO.aq, AMO.rl, AMO.aq.sc, and AMO.rl.sc. instructions
    
    \textbf{Refinement}: Done
\end{enumerate}

%\subsection{MCM Improvements}
%-- modify fences to be cumulative in baseline when they order writes before another write \\
%-- modifiy release operation to be cumulative \\
%-- modify sc operations to allow roach motel \\
%-- modify aquire and release operations so that only acquires can syncrhonize with a release, and not just any read \\

\begin{table}
\begin{center}
\centering
\small
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{| c | c | c |}
    \hline
    \textbf{Description}              & \textbf{Base} & \textbf{Base + A} \\ \hline
    ISA Manual~\cite{RISCV}  & base\_riscv         & baseA\_riscv             \\ \hline
    MCM Improvements        & base\_riscv+        & baseA\_riscv+            \\ 
\hline
\end{tabular}
\end{center}
\caption{For each of the RISC-V models detailed in Table~\ref{table:relaxations}, we implemented a number of versions. We began by implementing Base and Base + A versions based on the current ISA specification. We the made first-level improvements to the baseline version to improve accurracy and efficiency of mapping from C/C++. For the Base + A version only, we made second-level improvements that specifically affect \texttt{acq} and \texttt{rel} operations.}
\label{table:modelkey}
\end{table}

-- Explain why we are omitting consume
--  Mention how RISC-V BOOM Chip incoporates a loads and store buffer, therefore is succeptible to some of these details in addition to being OoO.

\begin{table}
\begin{center}
\centering
\small
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{| c | c | c |}

 \hline
 \multicolumn{3}{| c |}{\textbf{Intuitive C/C++ $\rightarrow$ RISC-V Compiler Mappings}} \\ \hline
 \textbf{C/C++ Atomic}  & \textbf{RISC-V}           & \textbf{RISC-V} \\
 \textbf{Instruction}   & \textbf{(Base)}           & \textbf{(Base + A)} \\ \hline
 \texttt{ld rlx}        & ld                        &  ld                    \\ \hline
 \texttt{ld acq}        & ld; f[r,m]                & {AMO.aq}   \\ \hline
 \texttt{ld sc}         & ld; f[r,m]                & {AMO.aq.rl}\\ \hline
 \texttt{st rlx}        & st                        & st                     \\ \hline
 \texttt{st rel}        & {f[m,w]}; st              & AMO.rl                 \\ \hline
 \texttt{st sc}         & {f[m,w]}; st; {f[m,w]}    & {AMO.aq.rl}   \\ \hline
 \texttt{fence acq}     & f[r,m]                    & {f[r,m]}      \\ \hline
 \texttt{fence rel}     & {f[m,w]}                  &  f[m,w]                   \\ \hline
 \texttt{fence acq\_rel}& {f[m,m]}                  & {f[m,m]}     \\ \hline
 \texttt{fence sc}      & {f[m,m]}                  & {f[m,m]}     \\ \hline
 Safety Net             & {f[m,m]}                  & {f[m,m]}     \\
 \hline
 
\end{tabular}
\end{center}
\caption{Intuitive compiler mappings from C/C++ to both the Base and Base + A versions of the RISC-V ISA. \textit{f[a,b]} designates a fence that orders accesses of type \textit{a} before the fence and accesses of type \textit{b} after the fence. Memory reads and writes are represented by \textit{r} and \textit{w}, respectively, and \textit{m} corresponds to any memory operation (i.e., read or write). \textit{AMO.a} designates an AMO operation with the \textit{a} bit set. The manual~\cite{RISCV} states that the \texttt{acq} and \texttt{rel} annotations for AMO operations were designed to implement the C11 and C++11 memory models efficiently. It additionally states that the f[r, m] suffices to implement an \texttt{acq} operation and f[m,w] suffices to implementat a \texttt{rel}. These mappings are derived from this information.}
\label{table:compilermappings}
\end{table}


%Method \\
%Make successive relaxations to a baseline to show a variety and study differences \\
%Determine what kinds of instructionss we need to restore PO/atomicity when we want to
%Based on the relaxations, what MOR is required to implment C++\\
%What does RISC-V supply, is it enought/efficient?

% \subsection{How can we evaluate performance?}
% We only need fences to enforce local orderings that are relaxed by hardware. Minimal requirement is a full fence. Extras are:
%     \begin{itemize}
%         \item Fences at finer granularity depending on re-orderings permitted by hardware.
%         \item SC acquire and release fences
%         \item Relaxed acquire and release fences
%     \end{itemize}
% \end{itemize}
% \textbf{If we know stores are multiple copy atomic:}
% \begin{itemize}
%     \item Need fences to enforce local 
% \end{itemize}We need a Store -> Load fence to flush the store buffer. A Store -> Store can be maintained if there is no coalescing in the write buffer; otherwise we need a flush here. Load -> Load and Load -> Store are simpler.
% TODO

% \subsection{What are the RISC-V implementations like?}
% \begin{itemize}
%     \item How is the cycle accurate simulator generated?
%     \begin{itemize}
%         \item Cycle accurate simulator generated by Chisel (LOOK AT OUTPUT FROM LAST TIME AGAIN)
%         \item Chisel can generate a fast C emulator from the scala source files that is handy for simulating and debugging hardware designs.
%         \item This will compile a C emulator capable of cycle-accurate simulation of the Rocket core.
%         \item The dramsim argument includes the simu- lated DRAM in the processor emulation. max-cycles sets a timeout constraint in case the program hangs. The loadmem command allows the program data to be loaded into simulated memory before the simulation begins. Without this command, numerous simulation cycles would be spent at the beginning of each program loading data into memory.
%         \item In Rocket, the program counter is always initialized to 0x2000, so our program starts there. You’ll notice that the program counter remains at this address for many cycles before any instructions are executed. This is because the memory system simulates a typical latency for DRAM accesses, which are required to load instructions into the cache before the processor can begin executing the program. Note the additional long pauses over the course of the program’s execution while the processor stalls, waiting for the results of memory requests. This is the main (though not the only) reason that simulations of programs run on the processor take many more simulated cycles than those run on spike
%         \item Is there a variable latency DRAM?
%     \end{itemize}
%     \item What does the pipeline of Rocket Chip look like?
%     \begin{itemize}
%         \item Rocket is an in-order, single-issue scalar processor that includes a six-stage integer pipeline. It has a 31-entry, 64-bit register file and uses a scoreboard to detect data hazards involving instructions with multi-cycle latencies.
%     \end{itemize}
%     \item What does the pipeline of BOOM look like?
%         \item Complex processor. Has a store queue, but is it better to make my own for the simpler Rocket Chip? Should only need to deal with Scala and Chisel.
% \end{itemize}

% \begin{itemize}
%     \item Use Pipecheck to model current RISC-V design (Rocket Chip)
%     \item Use simulator to determine performance of different implementation choices as elaborated above
%     \item Use Pipcheck to ensure that design modifications still prohibit certain litmus test outcomes
% \end{itemize}

\iffalse
begin{table*}
\begin{center}
\centering
\small
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{| c | c | c | c | c | c |}

 \hline
 \
 \textbf{C/C++ Instruction} & \textbf{Power}        & \textbf{ARMv7}    & \textbf{ARMv8}    & \textbf{RISC-V (Base)}    & \textbf{RISC-V (Base + A)} \\ \hline
 \texttt{ld rlx} & ld                   & ldr               & ldr   & ld                  &  ld                    \\ \hline
 \texttt{ld acq} & ld; cmp; bc; isync   & ldr; dmb          & lda   & ld; f[r,m]          & {\color{red} AMO.aq}   \\ \hline
 \texttt{ld sc}  & hwsync; ld; cmp; bc; isync& ldr; dmb     & lda   & ld; f[r,m]          & {\color{blue}AMO.aq.rl}\\ \hline
 \texttt{st rlx} & st                   & str               & str   & st                  & st                     \\ \hline
 \texttt{st rel} & lwsync;st            & dmb; str          & stl   & {\color{red}f[m,w]}; st & AMO.rl                 \\ \hline
 \texttt{st sc}  & hwsync; st           & dmb; str; dmb     & stl   & {\color{red}f[m,w]}; st & {\color{blue}AMO.aq.rl}   \\ \hline
 \texttt{fence acq} & lwsync            & dmb               & dmb   & f[r,m]              & {\color{red}f[r,m]}      \\ \hline
 \texttt{fence rel} & lwsync            & dmb               & dmb   & {\color{red}f[m,w]} & f[m,w]                   \\ \hline
 \texttt{fence acq\_rel} & lwsync       & dmb               & dmb   & {\color{red}f[m,m]} & {\color{red}f[m,m]}     \\ \hline
 \texttt{fence sc}  & ld                & ldr               & ldr   & {\color{red}f[m,m]} & {\color{red}f[m,m]}     \\ \hline
 Safety Net         & hwsync            & dmb               & dmb   & {\color{red}f[m,m]} & {\color{red}f[m,m]}     \\
 \hline
 
\end{tabular}
\end{center}
\caption{Possible compiler mappings from C/C++ to both the baseline (i.e., Base) and baseline-plus-atomics (i.e., Base + A) versions of RISC-V and to other ``weak'' ISAs~\cite{} (i.e., Power, ARMv7, adn ARMv8). The RISC-V mappings provided in this table represent what we believe to be the ISA designers' intended compiler mappings.}
\label{table:compilermappings}
\end{table*}
\fi


==> relaxations.tex <==
\section{Our Framework for MCM-Aware ISA Design}
\label{sec:method}
%Section 3 also probably needs a more explicit discussion of why a litmus-test based approach is OK (as opposed to complete coverage of every possible scenario). Litmus tests are intuitive and have been chosen by experts and represent a practical way to find many bugs early in the process. This framework is not a substitution for  more complete formal methods later in the design process, yada yada yada.

ISAs are designed somewhat frequently and evolve even more often. For example, ARM has recently added one-way acquire and release barriers to better accommodate the requirements of C/C++ atomics~\cite{armv8}. There is a window of opportunity in which ISA design and modification can take place prior to it being officially released as a target for compiler tool-chains and an implementation specification for hardware design. Inspired by the affects of weakening MCM features and potential issues that can arise in practice when ISA MCMs are inadequately specified, we have designed an iterative toolflow and methodology for ISA MCM evaluation and refinement, incorporating the subtle ways in which common microarchitectural optimizations manifest at the architecture level.

\subsection{Background: \textit{$\mu$Check} and \textit{Herd}}
Our approach is primarily based on the \textit{$\mu$Check}~\cite{pipecheck,ccicheck,coatcheck} family of tools. 
A hardware designer can use a DSL, \textit{$\mu$Spec}, to describe a processor by defining a set of ordering axioms. This specification along with a collection of user-provided litmus tests and corresponding required outcomes for each test serve as inputs to $\mu$Check. $\mu$Check evaluates correctness of the processor model by comparing the required litmus test outcomes with outcomes that are \textit{observable} on the model.

We use these tools alongside \textit{Herd}~\cite{alglave:herd}, 
%and use a Herd-to-$\mu$Check translation script to compare HLL-level and hardware-level execution scenarios. In particular, we automate the process of evaluating ISA specifications based on their ability to serve as viable compiler targets producing memory-model-compliant code for C/C++ programs.
a memory model simulator that takes as input a user-defined MCM (in a concise, specified format) and a litmus test and outputs all executions of that tests that are \textit{permitted} by the model.
%The original Herd framework included support solely for machine-level models of CPUs and GPUs.
Recent work has added support for language-level MCMs, and in particular, a model has been constructed for C/C++~\cite{batty:overhauling}.



\subsection{Iterative MCM-Aware ISA Design with $\mu$Check}
As depicted in Figure~\ref{fig:isa}, the ISA MCM specification is the contract between software and hardware that determines what orderings should be enforced by the hardware and which are the responsibility of the compiler to enforce by leveraging ISA instructions. 
In this work, we study focus on the time in the design process when the ISA MCM can be modified. 
%Furthermore, our ultimate test of ``correctness'' is the ability of an ISA MCM to provide the interface required for producing correct and efficient executions of C/C++ programs.
When the ISA MCM is a fluid design component, it becomes necessary to have the ability modify both microarchitecutral implementations of that ISA MCM as well as compiler mappings from C/C++ MCM primitives to the ISA MCM.

In this light, we selected the $\mu$Check framework to promote ISA MCM and microarchitecture co-design.
The $\mu$Check framework has been used in prior work as way to verify that a microarchitecture is correctly upholding the requirements of its corresponding ISA MCM~\cite{pipecheck, ccicheck, coatcheck}.
Here we show how one can leverage this framework to assist in determining if a specific combination of a C/C++$\rightarrow$ISA MCM \textit{compiler mapping}, an \textit{ISA MCM} specification, and a \textit{microarchitectural implementation} can prohibit all illegal-according-to-C/C++ executions and permit as many legal-according-to-C/C++ as possible (i.e., minimally constrain C/C++ programs).

$\mu$Check also demonstrates that subtle microarchitectural modifications may directly affect the ISA-level MCM, and consequently how it can (or cannot) serve as a compiler target for C/C++ programs. While architects are selecting hardware optimizations for improved performance or simplifications for ease of verification, they can simultaneously study the effects of these choices on the ISA-visible MCM and the ability of their design to accurately and efficiently support C/C++ programs.
$\mu$Check is a robust framework that enables designers model custom \textbf{TODO: heterogeneous} design as well as the interplay between coherence and consistency~\cite{ccicheck} and virtual memory and consistency~\cite{coatcheck}. Can do this instead of having ISA-visible insturction reordering 
$\mu$Check is also able to model the speculative techniques mentioned in Section~\ref{sec:background} by simply omitting incorrectly-speculated events its axiom evaluation~\cite{pipecheck}.



As depicted in Figure~\ref{fig:method} our iterative toolflow is as follows:
\begin{enumerate}
    \item \label{item:inputs} \textsc{Initial Inputs}:
        \begin{enumerate}
            \item A proposed \textit{ISA MCM} specification for evaluation.
            \item \textit{Compiler mappings} from C/C++ MCM primitives to the ISA's assembly instructions.
            \item A $\mu$Spec model corresponding to a \textit{microarchitectural implementation} of the ISA MCM.
        \end{enumerate}
    \item \label{item:ctests} \textsc{C/C++ Litmus Test Generation}: Starting from C/C++ litmus test templates (i.e., a Herd-style C/C++ litmus tests with placeholders for C/C++ \texttt{memory\_order} primitives), we generate all permutations of each test, featuring all combinations of applicable C/C++ \texttt{memory\_order} primitives. This allows us to verify ISA MCM functionality for all possible \texttt{memory\_order} interactions and synchronization scenarios for a given litmus test.
    \item \label{item:axiomatic} \textsc{C/C++ Axiomatic Evaluation}: The suite of C/C++ litmus tests is run on the C/C++ Herd model to determine the outcomes that the C/C++ HLL MCM \textit{permits} or \textit{forbids} for each at the program level.
    \item \label{item:compilation} \textsc{C/C++$\rightarrow$ISA Compilation}: Using the C/C++$\rightarrow$ISA compiler mappings, we generate a corresponding assembly version for each of the C/C+ litmus test permutations.
    \item \label{item:operational} \textsc{ISA $\mu$Spec Evaluation}: The suite of assembly litmus tests is run on the ISA $\mu$Check model to determine the outcomes that are \textit{observable} or \textit{unobservable} on the microarchitecture.
    \item \label{item:equivalence} \textsc{Operational-Axiomatic Equivalence Check}: The results of Step~\ref{item:axiomatic} and Step~\ref{item:operational} are compared for each test to determine if the microarchitecturally realizable outcomes are \textit{stronger than}, \textit{weaker than}, or \textit{equivalent to} the outcomes required by C/C++. A \textit{stronger than} (resp. \textit{weaker than}) outcome corresponds to a C/C++ program that is \textit{permitted} (resp. \textit{forbidden}) by the C/C++ MCM, yet \textit{unobservable} (resp. \textit{observable}) on the microarchitectural implementation of the ISA. If Step~\ref{item:equivalence} concludes that the microarchitecturally realizable outcomes are more restrictive than what C/C++ requires, the designer may wish to conduct refinement for performance reasons. On the other hand, refinement is \textit{mandatory} when outcomes forbidden by the C/C++ model are observable on the microarchitecture.
    \item \label{item:refinement} \textsc{Refinement}: This step corresponds to refining any combination of the \textit{ISA MCM}, \textit{compiler mappings}, and \textit{microarchitectural implementation}. \textit{Refinement} refers to the process of modifying an input in response to a microarchitectural implementation that differs from the C/C++-specified outcome for a given set of program executions. 
    %\item \label{item:iterate} \textsc{Iterate}: If no refinement is necessary or desired, exit the toolflow. Otherwise, return to Step~\ref{item:compilation} with the newly-refined components from Step~\ref{item:refinement}.
\end{enumerate}



\subsection{Microarchitectural Implementations}
%\textbf{TODO:} We use our framework on these microarchitectures, and as an exmple of ISAs here's RISV
\label{sec:microimplmentations}
%Throughout out our iterative refinement process, we modeled many RISC-V processor designs with varying levels of microarchitectural optimization.
%The initial stricter-than-required $\mu$Spec design (for both Base and Base~+~A) is a pipeline resembling Rocket Chip~\cite{rocketchip}, a 6-stage in-order pipeline that implements the Base RISC-V ISA as well as some optional extensions, including the Atomics extension discussed in Section~\ref{sec:riscv}.
%Step~\ref{item:refinement} indicates that any combination of compiler mappings, ISA MCM specification, or $\mu$Spec model, may be refined at the end of one iteration/start of another. On all iterations of our toolflow that involved a $\mu$Spec model refinement, all refinements resulting in microarchitectural ``weakenings'' were legal according to the current RISC-V ISA MCM specification.

\begin{table}
\begin{center}
\centering
\small
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{| l | c | c | c | c | c | c |}

 \cline{2-7}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Relaxed PO}} & \multicolumn{3}{c|}{\textbf{Store Atomicity}} \\ \hline
 \multicolumn{1}{|l|}{\textbf{RISC-V Model}} & W$\rightarrow$R & W$\rightarrow$W & R$\rightarrow$M & MCA & rMCA & nMCA \\ \hline
 WR     & \cm   &       &       & \cm   &       &       \\ \hline
 rWR    & \cm   &		&       &       & \cm   &       \\ \hline
 rWM	& \cm   & \cm   &       &       & \cm   &       \\ \hline
 rMM	& \cm	& \cm	& \cm   &       & \cm   &       \\ \hline
 nWR    & \cm   &       &		&       &       & \cm   \\ \hline
 nMM    & \cm	& \cm   & \cm	&       &    	& \cm   \\ \hline
 A9     & \cm	& \cm   & \cm	&       &    	& \cm   \\ 

 \hline
 
\end{tabular}
\end{center}
\caption{$\mu$Spec models constructed by relaxing various aspects of program and store atomicity. We note that these models exercise optimizations analogous to those presented in~\cite{adve:tutorial}.}
%\caption{RISC-V $\mu$Spec models constructed by relaxing various aspects of program and store atomicity from a baseline model resembling the RISC-V Rocket Chip~\cite{rocketchip}. All relaxations are legal according to the RISC-V ISA Manual~\cite{RISCV}. R, W, and M, correspond to read accesses, write accesses, and memory accesses (reads or writes), respectively. We note that these models exercise optimizations analogous to those presented in~\cite{adve:tutorial}.}
\label{table:relaxations}
\end{table}

To support our framework, we have assembled and implemented a set of microarchectures in $\mu$Spec that exploit a variety of program order (PO)


Table~\ref{table:relaxations} summarize the spectrum of RISC-V-allowed relaxations that we exploited in our refinement process for both halves of our evaluation. As the RISC-V ISA does not distinguish between same address and different address memory instruction orderings, we do not distinguish a difference in this table.
Initially, all relaxations were implemented by adding various combinations of memory access buffers after the Commit stage in the Rocket Chip pipeline. We achieve the relaxation combinations of Table~\ref{table:relaxations} as follows:
\begin{enumerate}
    \item \textbf{WR}: W$\rightarrow$R reordering is achieved by buffering stores in a FIFO queue prior to being eventually pushed out to the rest of the memory hierarchy. Younger loads may continue past pending stores as long as the load address does not match the address of a pending store in the store buffer. Whenever there is a match, the load must wait for the corresponding store (and any prior stores, due to the FIFO property of the queue) to reach the memory hierarchy before it can load any data. No core can read writes early, so stores are MCA.
    \item \textbf{rWR}: Builds on WR by allowing the store buffer to forward values pending store values to later loads of the same address. Later loads my proceed past earlier stores, regardless of their effective addresses. Stores preform once locally and again globally, rendering them rMCA.
    \item \textbf{rWM}: Extends rWR by allowing writes (to different addresses) to retire from the store buffer out of order. Coherence requires a total global order on stores to the same address.
    \item \textbf{rMM}: Extends rWM by allowing reads to commit out of order with earlier reads or writes. We maintain that read$\rightarrow$write ordering must be maintained for same address reads and writes, but we allow reordering for all read$\rightarrow$read pairs as the specification does not specify any particular ordering semantics for reads of the same address.
    \item \textbf{WR+nMCA}: Extends rWR by allowing cores to share store buffers. This is analogous to the shared write-through cache scenario of \cite{cppconcurrency}, and enables nMCA stores.
    \item \textbf{nMM}: Extends rMM by allowing shared store buffers in the same vein as nWR.
    \item \textbf{A9}: To demonstrate that the intricacies of nMCA stores do not depend on a design that contains a shared buffer or shared write-through cache, we model another microarchitecture with ISA-visible relaxations that match those of nMM. This time we leverage the ability of $\mu$Check to model the subtleties that can arise a the cache-coherence-consistency interface. To implement nMCA stores, this model features a write-back cache that allows multiple requests for write permission (for different addresses) to be in progress at the same time and a non-stalling directory protocol that allows the storing core to forward the store's value to another core before it has received all in validations for the access. In this scenario, coherence is preserved, but nMCA stores arise~\cite{}.
    \textbf{TODO}: Mention SWMR and DVI? Or desribe \textit{why} coherence is preserved?
\end{enumerate}
%\subsection{Iterative MCM-AWARE ISA Refinement}

%As a preliminary test of this framework, we took the C++ coRSDWI litmus test of Figure~\ref{fig:motivating} and ran it on the C/C++ Herd model. As expected, the outcome of this test indicated that the two consecutive loads of \texttt{z} on \texttt{Core 0}, cannot can never hold return the values 2 and 1, respectively. We implemented a $\mu$Spec model of the ARM Cortex-A9 processor core, referencing public documentation~\cite{}, and ran the ARM assembly version of coRSDWI from Fiture~\ref{fig:motivating} on model. The result of of this test is depicted in  Figure~\ref{fig:coRSDWIgraph}. 


